Object2Scene: Putting Objects in Context for Open-Vocabulary 3D Detection

Point cloud-based open-vocabulary 3D object detection aims to detect 3D categories that do not have ground-truth annotations in the training set. It is extremely challenging because of the limited data and annotations (bounding boxes with class labels or text descriptions) of 3D scenes. Previous approaches leverage large-scale richly-annotated image datasets as a bridge between 3D and category semantics but require an extra alignment process between 2D images and 3D points, limiting the open-vocabulary ability of 3D detectors. Instead of leveraging 2D images, we propose Object2Scene, the first approach that leverages large-scale large-vocabulary 3D object datasets to augment existing 3D scene datasets for open-vocabulary 3D object detection. Object2Scene inserts objects from different sources into 3D scenes to enrich the vocabulary of 3D scene datasets and generates text descriptions for the newly inserted objects. We further introduce a framework that unifies 3D detection and visual grounding, named L3Det, and propose a cross-domain category-level contrastive learning approach to mitigate the domain gap between 3D objects from different datasets. Extensive experiments on existing open-vocabulary 3D object detection benchmarks show that Object2Scene obtains superior performance over existing methods. We further verify the effectiveness of Object2Scene on a new benchmark OV-ScanNet-200, by holding out all rare categories as novel categories not seen during training.

==> figures/fig_pipeline.tex <==
\begin{figure*}[t]
  \centering
   \includegraphics[width=0.72\linewidth]{imgs/pipeline.png}
   \captionsetup{aboveskip=0pt}\captionsetup{belowskip=0pt}\caption{Overall pipeline for our model. It consists of an visual encoder, a text encoder and our own designed Uni-Decoder.} 
   \label{fig:pipeline}
\end{figure*}   

==> figures/fig_querycontrast.tex <==
\begin{figure*}[t]
  \centering
   \includegraphics[width=0.72\linewidth]{imgs/query_contrast.png}
   \captionsetup{aboveskip=0pt}\captionsetup{belowskip=0pt}\caption{Illustration of Query-level Contrast. For each scene, the GTs which belong to the same category (green) and GTs of other categories (gray) are constructed to be positive/negative pairs. The contrastive loss is applied to all positive and negative GT pairs based on their feature  similarities. Since the GTs may come from different dataset domain, we can reduce the domain gap by contrastive learning.} 
   \label{fig:qc}
\end{figure*}   

==> tables/table_contrastive.tex <==
\begin{table}
\caption{Analysis of contrastive learning.}
  \centering
  % \scriptsize
  \resizebox{0.36\linewidth}{!}{
  \begin{tabular}{lc}
    \toprule
    Transfer direction & $mAP_{25}$ \\
    \midrule
    ScanNet -> ScanNet      & 25.6   \\
    ScanNet -> SUN RGB-D    & 16.3   \\
    SUN RGB-D -> SUN RGB-D  &   \\
    SUN RGB-D -> ScanNet  &   \\
    \bottomrule
  \end{tabular}
  }
  \label{tab:trans}
  \vspace{-0.2cm}
\end{table}

==> tables/table_diversity.tex <==
\begin{table}
  \centering
  % \scriptsize
  \resizebox{0.56\linewidth}{!}{
  \begin{tabular}{lcc}
    \toprule
    3D object dataset & overlap $mAP_{25}$ & $mAP_{25}$ \\
    \midrule
    ShapeNet      &  7.87  &11.21   \\
    \chenming{OmniObject3D}  & 11.31 & 16.92   \\
    ShapeNet + \chenming{OmniObject3D}  & 15.67  & 24.62 \\
    \bottomrule
  \end{tabular}
  }
  \caption{Analysis of 3D object diversity. overlap $mAP_{25}$ represents the mean $AP_{25}$ on the overlap classes of ShapeNet and ScanobjectNN in OV-ScanNet20 benchmark.}
  \label{tab: diversity}
  \vspace{-0.2cm}
\end{table}

==> tables/table_overall.tex <==
\begin{table}
  \centering
  % \scriptsize
  \resizebox{0.36\linewidth}{!}{
  \begin{tabular}{lc}
    \toprule
    Transfer & $mAP_{25}$ \\
    \midrule
    ScanNet -> ScanNet      & 25.6   \\
    ScanNet -> SUN RGB-D    & 16.3   \\
    SUN RGB-D -> SUN RGB-D  &   \\
    SUN RGB-D -> ScanNet  &   \\
    \bottomrule
  \end{tabular}
  }
  \caption{Analysis of contrastive learning.}
  \label{tab:trans}
  \vspace{-0.2cm}
\end{table}

==> tables/table_prompts_type.tex <==
\begin{table}
  \centering
  % \scriptsize
  \resizebox{0.36\linewidth}{!}{
  \begin{tabular}{lc}
    \toprule
    Prompt type & $mAP_{25}$ \\
    \midrule
    Detection Prompt      & 14.91   \\
    Absolute Location Prompt    & 17.42   \\
    Relative Location Prompt  & 21.31 \\
    \bottomrule
  \end{tabular}
  }
  \caption{Analysis of text prompts used in Object2Scene prompt generation.}
  \label{tab:prompt_type}
  \vspace{-0.2cm}
\end{table}

==> tables/table_scannet200.tex <==
\begin{table}[t!]
  \centering
  % \scriptsize
  \resizebox{0.22\linewidth}{!}{
  \begin{tabular}{lcc}
    \toprule
    Method  & common & tail \\
    \midrule
    L3Det     & 10.1 & 3.4  \\
    \bottomrule
  \end{tabular}
  }
  \caption{Detection results on OV-ScanNet200 benchmark.}
  \label{tab:scannet200}
  \vspace{-0.2cm}
\end{table}

==> tables/table_transferability.tex <==
\begin{table}
  \centering
  % \scriptsize
  \resizebox{0.36\linewidth}{!}{
  \begin{tabular}{lc}
    \toprule
    Transfer direction & $mAP_{25}$ \\
    \midrule
    ScanNet -> SUN RGB-D    & 16.34   \\
    SUN RGB-D -> ScanNet  & 17.11  \\
    \bottomrule
  \end{tabular}
  }
  \caption{Analysis of transferability.}
  \label{tab:trans}
  \vspace{-0.2cm}
\end{table}
